Stationary solutions of driven fourth- and sixth-order Cahn-Hilliard type equations

New types of stationary solutions of a one-dimensional driven sixth-order Cahn-Hilliard type equation that arises as a model for epitaxially growing nano-structures such as quantum dots, are derived by an extension of the method of matched asymptotic expansions that retains exponentially small terms. This method yields analytical expressions for far-field behavior as well as the widths of the humps of these spatially non-monotone solutions in the limit of small driving force strength which is the deposition rate in case of epitaxial growth. These solutions extend the family of the monotone kink and antikink solutions. The hump spacing is related to solutions of the Lambert $W$ function. Using phase space analysis for the corresponding fifth-order dynamical system, we use a numerical technique that enables the efficient and accurate tracking of the solution branches, where the asymptotic solutions are used as initial input. Additionally, our approach is first demonstrated for the related but simpler driven fourth-order Cahn-Hilliard equation, also known as the convective Cahn-Hilliard equation.

==> app-kappap-CCH.tex <==
\section{ Region near $\boldsymbol\kappa_p$}
\label{app-kappap-CCH}
%\paragraph{Region near $\boldsymbol\kappa_p$} 

As for the region near $\kappa_m$, here we stretch the variable as 
\be
x_p=\frac{x-\bar\kappa_p}{\sqrt{2}\,\eps},\mywhere \bar\kappa_p>0 \label{xp}
\ee
and set
\be
\kappa_p=\bar\kappa_p +\sqrt{2}\,\eps\sum^{\infty}_{k=1}\delta^k \kappa_{pk}
\label{kappap}
\ee
We write the solutions as 
\be
u(\bar\kappa_p+\sqrt{2}\,\eps\,x_p; \eps)= u_p(x_p; \eps)\label{up}
\ee
The so transformed governing equation becomes
\be
u_p'''+2(u_p-u_p^3)'=\sqrt{2}\,\delta(\eps)\,(u_p^2-A)\mywhere \prime=\frac{d}{dx_p}\label{cchp}
\ee
For the boundary conditions we place $\kappa_p$ near the point, where 
$u_p$ crosses zero, i.e. 
\be
u_p\left(\frac{\kappa_p-\bar\kappa_p}{\sqrt{2}\,\eps}\right) = 0
\label{upbc0}
\ee
and the condition towards $\infty$ is 
\be
\lim_{x_p\to \infty} u_p(x_p)=-\sqrt{A}.
\label{cchpbc0}
\ee

We assume $u_p(x_p)$ can be written as the following asymptotic expansion, 
valid near $\kappa_p$
\be
u_p(x_p; \eps) = u_{p0}(x_p) + \sum_{k=1}^{\infty}\delta^k(\eps)\, u_{pk}(x_p)
\label{upexp}
\ee

To leading order in $\delta(\eps)$ we get the problem 
\sbea\label{leadup}
\begin{align}
&u_{p0}'''+ 2(u_{p0} - u_{p0}^3)'=0\\
&u_{p0}(0)=0\myand \lim_{x_p\to \infty} u_{p0}(x_p) = -1
\end{align}
\seea
A solution is 
\be
u_{p0}(x_p)=-\tanh(x_p)
\ee
The equation of order $\delta(\eps)$ is 
\sbea\label{up1}
\begin{align}
&\Big(u_{p1}''+ 2\left(1 - 3\tanh^2(x_p)\right)\,u_{p1}\Big)'=\sqrt{2}\,\left(\tanh^2(x_p)-1\right)\\
&u_{p1}(0)=\kappa_{p1}\myand \lim_{x_p\to \infty} u_{p1}(x_p) = -\frac{A_1}{2}
\end{align}
\seea
Integrating \rf{up1} once yields 
\be
u_{p1}''+2\left(1-3\tanh^2(x_p)\right)\,u_{p1}= f_p(x_p)
\ee
where 
\be
f_p(x_p)=-\sqrt{2}\left(\tanh(x_p)-1\right) + 2A_1
\ee
The general solution is 
\be
u_{p1}(x_p)= \kappa_{p1}\,\phi_{{p}_{1}}(x_p)+\phi_{{p}_{i}}(x_p)\label{solup1}
\ee
where the homogeneous and inhomogeneous solutions are here 
\sbea
\begin{align}
\phi_{{p}_{1}}(x_p)&= u_{p0}'(x_p)\myand \phi_{{p}_{2}}(x_p) =  \left(\int^{x_p}_0\frac{dz}{\phi^2_{{p}_{1}}(z)}\right)\phi_{{p}_{1}}(x_p)  \label{phip12}\\
\phi_{{p}_{i}}(x_p)&=-\phi_{{p}_{2}}(x_p)\int_{x_0}^{\infty}\,\phi_{{p}_{1}}\,f_p\,dz - \phi_{{p}_{1}}(x_p)\int_{0}^{x_p}\,\phi_{{p}_{2}}\,f_p\,dz    \label{phipi}
\end{align}
\seea
Note that the inhomogeneous solution 
is normalized such that $\phi_{{p}_{i}}(0)=0$ and $\lim_{x_p\to\infty}\phi_{{p}_{i}}(x_p)$ remains bounded. 



==> comparison-hcch.tex <==
This result for $A_1$ compares well with numerical results for the 
coefficient. 
We observe also that a fit to the numerical solution for $A_1$ for 
a $2$-hump solution should be $A_1=5\,2^{1/6}$. These relations 
are very analogous to the results for CCH. 

\subsection{Asymptotic solution}

\begin{figure}%[p]
\centering
\includegraphics*[width=0.6\textwidth]{Eps/het-comparison.eps}
\caption{\label{compareA1}Comparison of $A_1$ with numerical results,for $\delta= 0.00038152$} 
\end{figure}


==> makefile <==
#$Id: makefile,v 1.5 2005/03/13 19:30:35 amue Exp $

PDF_PREFIX=HCCH-
LATEX=latex -src -shell-escape

do:	paper.dvi

	
paper.ps: paper.dvi
	dvips  paper.dvi -Pcmz -Pamz -o paper.ps

paper2up.ps: paper.ps
#	pstops '2:0L@.78(21.5cm,-.5cm)+1L@.78(21.5cm,14.35cm)' paper.ps > paper2up.ps
	psnup -2 paper.ps > paper2up.ps
	pstops '4:0L@.7(21cm,0)+1L@.7(21cm,14.85cm),2R@.7(0,29.7cm)+3R@.7(0cm,14.85cm)' \
		paper.ps > paper2up_stdhu.ps

tag-pdf: clean paper.dvi
	sh -x -c 'TAG=`date +%Y_%h%d_%T`; dvips -Ppdf paper.dvi -o - | ps2pdf - ${PDF_PREFIX}$${TAG}.pdf'

#tag-wias: clean paper.dvi
#	sh -x -c 'TAG=`date +%Y_%h%d_%T`; dvips -Ppdf paper.dvi -o ${WIAS_PREFIX}$${TAG}.ps; ps2pdf  ${WIAS_PREFIX}$${TAG}.ps ${WIAS_PREFIX}$${TAG}.pdf; bzip2 ${WIAS_PREFIX}$${TAG}.ps'

arch: paper.ps
	rm -rf transfer
	mkdir transfer
	cp paper.tex transfer
	cp stb-ridge-bib.bib transfer
	cp paper.bbl transfer
	cp paper.blg transfer
	( eps_files=`awk '/File:.*type eps)/{print $$2}' paper.log |sort`; \
	  cp $$eps_files transfer )
	sh -x -c 'TAG=`date +%h%d_%Y`; ps2pdf paper.ps dew_$${TAG}.pdf; cp dew_$${TAG}.pdf transfer'


paper.dvi: paper.tex hcch.bib macros.tex\
                intro.tex \
		paper.tex  \
		asymp-cch.tex 
	 ${LATEX} paper.tex
	 @( touch paper.toc; \
	      s=`cksum paper.toc`; \
	      while [ "$$s"  !=  "`cksum paper.toc`" ];	\
	      do  \
	              s=`cksum paper.toc`; \
	              ${LATEX} paper.tex>&/dev/null; \
	      done ; \
	      )
#	      ${LATEX} paper.tex;  )
	  @( if [ slip.bib -nt paper.tex ] ; then bibtex paper; ${LATEX} paper>&/dev/null; fi )
	  @( if (grep 'LaTeX Warning: There were undefined references' paper.log) ; then bibtex paper; ${LATEX} paper>&/dev/null; fi )
	  @( if (grep 'natbib Warning: There were undefined citations' paper.log) ; then bibtex paper; ${LATEX} paper>&/dev/null; fi )
	  @( while (grep 'Rerun to get cross-references right' paper.log); do ${LATEX} paper.tex >&/dev/null; done  )
	  @( while (grep 'Rerun to get citations correct' paper.log); do ${LATEX} paper.tex >&/dev/null; done  )
	  @( if (grep 'LaTeX Warning: There were undefined references' paper.log) ; then ${LATEX} paper>&/dev/null; fi )
#	  @( if (grep 'natbib Warning: There were undefined citations' paper.log) ; then ${LATEX} paper>&/dev/null; fi )
#	  @( if (grep 'natbib Warning: There were undefined citations' paper.log) ; then ${LATEX} paper>&/dev/null; fi )
#	  @( if (grep '(lineno)  	      rerun to get it right.' paper.log) ; then ${LATEX} paper>&/dev/null; fi )
	  @( if (grep 'LaTeX Warning: There were undefined references' paper.log) ; then ${LATEX} paper>&/dev/null; fi )
#	  @( if (grep 'natbib Warning: There were undefined citations' paper.log) ; then ${LATEX} paper>&/dev/null; fi )
#	  @( if (grep '(lineno)  	      rerun to get it right.' paper.log) ; then ${LATEX} paper>&/dev/null; fi )


#Eps/mrim-slip-top-ev.eps: Figs/mrim-slip-top-ev.agr
	xmgrace  -hardcopy -hdevice EPS  -printfile Eps/mrim-slip-top-ev.eps Grace/mrim-slip-top-ev.agr

#Eps/mrim-slip-bottom-ev.eps: Figs/mrim-slip-bottom-ev.agr
	xmgrace  -hardcopy -hdevice EPS  -printfile Eps/mrim-slip-bottom-ev.eps Grace/mrim-slip-bottom-ev.agr

#Eps/mrim-slip-longwave.eps: Figs/mrim-slip-longwave.agr
	xmgrace  -hardcopy -hdevice EPS  -printfile Eps/mrim-slip-longwave.eps Grace/mrim-slip-longwave.agr

#Eps/mrim-slip-ef.eps: Figs/mrim-slip-ef.agr
	xmgrace  -hardcopy -hdevice EPS  -printfile Eps/mrim-slip-ef.eps Grace/mrim-slip-ef.agr

#Eps/k-vs-shift.eps: Figs/k-vs-shift.agr
	xmgrace  -hardcopy -hdevice EPS  -printfile Eps/k-vs-shift.eps Grace/k-vs-shift.agr

#Eps/baseslip.eps: Figs/baseslip.agr
	xmgrace  -hardcopy -hdevice EPS  -printfile Eps/baseslip.eps Grace/baseslip.agr

.DELETE_ON_ERROR: paper.ps paper.dvi

.SUFFIXES: .agr .fig .eps

.agr.eps:
	xmgrace  -hardcopy -hdevice EPS  -printfile $@ $< 
#	xmgrace  -hardcopy -hdevice EPS  -printfile $@ $< -pexec 'with g0; legend off'
	
.fig.eps:
	fig2dev -L eps $< >  $@
bib:
	bibtex paper
	rm paper.dvi

clean:
	-rm *.dvi *.aux *.log 
	-rm o.pcl er.pcl all.pcl
	-rm paper.toc

veryclean: clean
	-rm paper.ps paper2up.ps ${PDF_PREFIX}*.pdf
	-rm paper.bbl paper.blg
	-rm *.bak
	
dep: 
	-${LATEX} '\scrollmode\input paper.tex'
	cp makefile makefile.bak
	awk '{print $0} /^# DO NOT DELETE/{exit}' makefile.bak >makefile
	-grep includegraphics paper*.tex |grep eps >temp-dep.log
	-grep 'File:.*type eps)' paper.log >>temp-dep.log
	echo paper.dvi: `awk '/File:.*type eps)/{print $$2}' temp-dep.log |sort -u` >>makefile 
	rm temp-dep.log
	
# DO NOT DELETE
paper.dvi: Eps/baseslip.eps Eps/k-vs-shift.eps Eps/mrim-slip-bottom-ev.eps Eps/mrim-slip-ef.eps Eps/mrim-slip-longwave.eps Eps/mrim-slip-top-ev.eps

